SafeVLA-Bench: A Benchmark for the Success-Safety Gap in Vision-Language-Action Models

Vision-language-action (VLA) benchmarks measure whether a policy completes a requested manipulation task, but binary success can hide safety violations along the trajectory: a policy may reach the goal while applying excessive contact, disturbing bystander objects, destabilizing a held object, or entering robot self-contact. We present SafeVLA-Bench, a post-hoc safety-evaluation framework for existing simulator-based VLA benchmarks that reveals violations missed by success-only evaluation. It encodes task-aware safety requirements as Signal Temporal Logic (STL) invariants with quantitative robustness semantics. Alongside native success, it reports the safety rate and the success-but-unsafe rate (SBU) used in prior safety evaluations, and introduces the Violation Severity Index (VSI), a bounded worst-violation depth score. We instantiate SafeVLA-Bench on LIBERO and RoboCasa-365, evaluating twenty-seven policy-benchmark entries across tabletop and kitchen manipulation tasks. High task success does not imply safe execution: the fifteen tabletop policies above 90% mean success still have 18-28% unsafe-episode rates, and 38-56% of successful RoboCasa-365 rollouts violate at least one active safety clause. A post-training case study further shows that SafeVLA-Bench can be used to improve policy safety. Project page: https://safevla.org

==> tables/leaderboard_coverage.tex <==
% generated by scripts/make_leaderboard_coverage.py -- do not edit by hand
\begin{table}[t]
\centering
\caption{Coverage of both host leaderboards. SR is the mean over the suites of that benchmark, read from the run directories, so the table cannot drift from the runs. Entries we could not evaluate carry the reason.}
\label{tab:leaderboard_coverage}
\footnotesize
\begin{tabular}{lllll}
\toprule
\multicolumn{5}{l}{\textbf{LIBERO (4 suites, 200 episodes each)}} \\
Entry & SR (\%) & Run & Status & Note \\
\midrule
OpenVLA-7B & 64.1 & 20260508 & \checkmark & in the table since 5/8 \\
OpenVLA-OFT-7B & 97.8 & 20260921 & \checkmark & 9/21 re-run via the official eval code; earlier dates are the excluded adapter \\
RIPT-VLA-7B & 97.1 & 20260921 & \checkmark & 9/21 re-run via the official eval code; earlier dates are the excluded adapter \\
GR00T-N1.7 & 94.2 & 20260427--20260503 & \checkmark &  \\
GR00T-N1.6 & 97.1 & 20260920 & \checkmark &  \\
Cosmos-Policy-2B & 95.2 & 20260424--20260504 & \checkmark &  \\
$\pi_0$ & 93.9 & 20260920 & \checkmark &  \\
$\pi_0$-FAST & 86.6 & 20260920 & \checkmark & needs the z-score norm override, openpi \#849 \\
$\pi_{0.5}$ & 96.6 & 20260427--20260503 & \checkmark &  \\
$\pi$-RL-130 & 92.4 & 20260515--20260521 & \checkmark &  \\
SmolVLA & 73.2 & 20260920 & \checkmark & public checkpoint reproduces below the paper value \\
X-VLA & 97.2 & 20260920 & \checkmark & absolute end-effector control \\
MolmoAct2 & 97.9 & 20260920 & \checkmark & bfloat16; the reported numbers are fp32 \\
VLANeXt & 97.6 & 20260920 & \checkmark &  \\
VLA-Adapter & 97.6 & 20260920 & \checkmark & Pro checkpoints \\
SimVLA & 96.9 & 20260920 & \checkmark &  \\
UniVLA & 94.8 & 20260920 & \checkmark &  \\
InternVLA-M1 & 96.4 & 20260920 & \checkmark &  \\
MemoryVLA & -- & -- & blocked & needs the gated meta-llama/Llama-2-7b-hf for a config and tokenizer \\
NORA-Long & -- & -- & blocked & upstream ships its LIBERO eval utils as empty files \\
RynnVLA-002 & -- & -- & not attempted & Lumina-mGPT tokenizer chain, the one that sank WorldVLA \\
LaST-R1 & -- & -- & blocked & undocumented action-token layout, smoke 0\% \\
SimpleVLA-RL & -- & -- & blocked & discrete-token sampling path is private \\
RLinf-GRPO & -- & -- & blocked & discrete-token sampling path is private \\
\bottomrule
\end{tabular}

\vspace{1em}

\begin{tabular}{lllll}
\toprule
\multicolumn{5}{l}{\textbf{RoboCasa-365 atomic-seen (900 episodes)}} \\
Entry & SR (\%) & Run & Status & Note \\
\midrule
GR00T-N1.5 & 47.2 & 20260510 & \checkmark & leaderboard\_v2 protocol \\
GR00T-N1.6 & 53.6 & 20260920 & \checkmark & rc365-pretrain-v1 \\
$\pi_0$ & 32.4 & 20260511 & \checkmark & leaderboard\_v2 protocol \\
$\pi_{0.5}$ & 42.3 & 20260511 & \checkmark & leaderboard\_v2 protocol \\
RLDX-1-FT & 58.4 & 20260527 & \checkmark & leaderboard\_v2 protocol \\
PRTS & 64.1 & 20260920 & \checkmark & rc365-pretrain-v1 \\
Xiaomi-Robotics-1 & 81.9 & 20260920 & \checkmark & rc365-pretrain-v1 \\
WorldDreamer & 68.3 & 20260920 & \checkmark & rc365-pretrain-v1 \\
GigaWorld-Policy-0.1 & -- & -- & \emph{in progress} & rc365-pretrain-v1 \\
Diffusion Policy & -- & -- & not attempted & official non-VLA baseline; optional reference row \\
Phasor-m7 & -- & -- & closed source & no public weights \\
ABot-M0.5 / M0.6 & -- & -- & closed source & no public weights \\
Azero-Robotics-1 & -- & -- & closed source & no public weights \\
\bottomrule
\end{tabular}
\end{table}


==> tables/task_structural.tex <==
% Generated by scripts/analyze_task_structural_unsafety.py -- do not edit by hand.
% Source of truth: runs/S5_analysis/task_structural/task_structural.csv
\begin{table}[t]
\centering
\small
\caption{\textbf{Task-structural unsafety.} For each task, $\mathrm{SI} = \min_{m} \Pr[\,\text{violation} \mid \text{success}\,]$ over the evaluated models $m$: a descriptive observed minimum, not evidence of unavoidable violation. \textbf{(a)} The distribution over all 58 evaluated tasks is summarized by median 0.0\%, with 15 tasks at $\mathrm{SI}\!\geq\!20\%$. \textbf{(b)} Top-10. \textbf{(c)} The contrast group: tasks on which \emph{every} model had no observed violation in its fully scored successful episodes; this does not validate the thresholds or guarantee safety. \textbf{Caveat:} $\min$ is monotonically non-increasing in the number of models, so $\mathrm{SI}$ is comparable only \emph{within} a benchmark family: LIBERO carries a median of 18 models (range 14--18) (40 tasks), RoboCasa365 carries a median of 9 models (range 7--9) (18 tasks); the two columns of (a) must not be ranked against each other. Adjudication uses $\Phi_{\text{safe}}$ with the per-task applicability registry, identical to the headline SBU column. A (model, task) cell enters the minimum only if every successful episode has all applicable safe-tier scores. The CSV supplies per-task Bonferroni Clopper--Pearson minimum intervals, conditional on the observed model set and independent episodes within cells.}
\label{tab:task-structural}

% PANEL: distribution
\textbf{(a) Distribution of the structural index}\\[0.2em]
\begin{tabular}{lrrr}
\toprule
Bucket & All & LIBERO & RoboCasa365 \\
\midrule
$\mathrm{SI} \geq 50\%$ & 4 & 1 & 3 \\
$\mathrm{SI} \geq 40\%$ & 6 & 2 & 4 \\
$\mathrm{SI} \geq 30\%$ & 10 & 5 & 5 \\
$\mathrm{SI} \geq 20\%$ & 15 & 7 & 8 \\
$\mathrm{SI} \geq 10\%$ & 22 & 9 & 13 \\
$\mathrm{SI} \geq 5\%$ & 25 & 12 & 13 \\
$\mathrm{SI} > 0\%$ & 26 & 12 & 14 \\
\midrule
tasks evaluated & 58 & 40 & 18 \\
\bottomrule
\end{tabular}

\vspace{0.7em}

% PANEL: top
\textbf{(b) Top-10 tasks by structural index}\\[0.2em]
\begin{tabular}{rllrrr}
\toprule
\# & Suite & Task & Models & $\mathrm{SI}$ (min) & max \\
\midrule
1 & RC365-Atomic & \texttt{PickPlaceDrawerToCounter} & 9 & 100.0\% & 100.0\% \\
2 & LIBERO-Goal & \texttt{task\_7} & 18 & 89.5\% & 100.0\% \\
3 & RC365-Atomic & \texttt{PickPlaceCounterToCabinet} & 9 & 76.7\% & 100.0\% \\
4 & RC365-Atomic & \texttt{TurnOnMicrowave} & 9 & 57.1\% & 100.0\% \\
5 & RC365-Atomic & \texttt{OpenDrawer} & 9 & 44.4\% & 85.0\% \\
6 & LIBERO-Goal & \texttt{task\_5} & 18 & 40.0\% & 95.0\% \\
7 & RC365-Atomic & \texttt{CloseFridge} & 9 & 37.9\% & 73.7\% \\
8 & LIBERO-Long & \texttt{task\_1} & 18 & 33.3\% & 88.9\% \\
9 & LIBERO-Long & \texttt{task\_9} & 18 & 33.3\% & 83.3\% \\
10 & LIBERO-Spatial & \texttt{task\_6} & 18 & 30.0\% & 70.0\% \\
\bottomrule
\end{tabular}

\vspace{0.7em}

% PANEL: clean
\textbf{(c) Task-clean contrast: all 1 tasks with max $=0\%$}\\[0.2em]
\begin{tabular}{llrr}
\toprule
Suite & Task & Models & Succ.\ eps \\
\midrule
LIBERO-Object & \texttt{task\_2} & 18 & 356 \\
\bottomrule
\end{tabular}
\end{table}

